MIDMs: Matching Interleaved Diffusion Models for Exemplar-based Image Translation

We present a novel method for exemplar-based image translation, called matching interleaved diffusion models (MIDMs). Most existing methods for this task were formulated as GAN-based matching-then-generation framework. However, in this framework, matching errors induced by the difficulty of semantic matching across cross-domain, e.g., sketch and photo, can be easily propagated to the generation step, which in turn leads to degenerated results. Motivated by the recent success of diffusion models overcoming the shortcomings of GANs, we incorporate the diffusion models to overcome these limitations. Specifically, we formulate a diffusion-based matching-and-generation framework that interleaves cross-domain matching and diffusion steps in the latent space by iteratively feeding the intermediate warp into the noising process and denoising it to generate a translated image. In addition, to improve the reliability of the diffusion process, we design a confidence-aware process using cycle-consistency to consider only confident regions during translation. Experimental results show that our MIDMs generate more plausible images than state-of-the-art methods.

==> 0_abstract.tex <==
\begin{abstract}
 We present a novel method for exemplar-based image translation, called matching interleaved diffusion models (MIDMs). Most existing methods for this task are roughly divided into two stages; matching and GANs-based generation. However, such matching-then-generation framework can hinder a faithful generation if unreliable correspondences are established. Motivated by the recent success of diffusion models, overcoming the shortcomings of GANs, we for the first time incorporate the diffusion models for this task. Specifically, we interleave cross-domain matching and diffusion steps in the latent space by iteratively feeding the intermediate warp into the noising process and denoising it to generate a translated image. In addition, to improve the reliability of diffusion process, we design confidence-aware process using cycle-consistency to consider only confident regions during translation.
 Experimental results show that our MIDMs generate more plausible images than state-of-the-art methods.
 

 
%  Warping exemplar images to align a given conditional input is a highly important process in exemplar-based translation tasks.  Unlike existing exemplar-based image translation works that separate two stages, the warping stage and GAN based generation stage, in that hinder a faithful generation if ill-warped indermediate is forwareded, MIDMs incorporates the warping process into the iterative denoising regime of diffusion models in a interactive manner, which highly boosts the performances. Specifically, we warp exemplar images to align conditional images and forward to diffusion network by adding proper amount of noise to refine warped images. We then interleave our in-domain alignment module in iterative denoising process.
%  Our in-domain alignment module newly warps the exemplar image using the refined warped image, capturing details of exemplar image faithfully while maintaining the alignment of conditional image. Interleaved in-domain alignment process proceeds in aware of confidence, so that adopting only reliable areas during iteretive warping. We conduct experiments to demonstrate the effectiveness of the proposed framework. MIDMs shows competitive quantitative performance while exhibiting superior qualitative results compared with state-of-the-art.
% RCD subdivides finding cross-domain correspondence into cross-domain warping and recurrent inter-domain warping processes.
\end{abstract}

==> Table/deepfashion_style.tex <==
% \renewcommand\arraystretch{1.0}
\begin{wraptable}{r}{0.5\textwidth}
% \,
\vspace{-3em}
\caption{\textbf{Quantitative evaluation of style relevance and semantic consistency on DeepFashion~\cite{}.}}
\label{tab_fashion_consistency}
\vspace{-5pt}
\small  
% \renewcommand\tabcolsep{8pt}
\centering 
\begin{tabular}{
lccc
} 
\toprule
\multirow{2}[3]{*}{Methods} & 
\multicolumn{2}{c}
{
Style relevance
} & 
\multirow{2}[3]{*}{\shortstack[c]{Semantic \\ consistency}}
\\
\cmidrule{2-3}
& Color & Texture &  \\
\midrule
Pix2PixHD~\cite{Wang2018HighResolution}    & -   &  -  & 0.914 \\

SPADE~\cite{park2019semantic}  &   0.955 &  0.927  & 0.922  \\

% SEAN~\cite{zhu2020sean} &  0.932     & 0.926 &  \multicolumn{2}{c}{0.860}  \\ 

% UNITE~\cite{zhu2017unpaired} & 0.963 & 0.945 &  \multicolumn{2}{c}{0.869} \\
MUNIT~\cite{huang2018multimodal} & 0.939 & 0.884 &  0.848 \\

EGSC-IT~\cite{ma2018exemplar} & 0.965 & 0.942 &  0.915 \\

CoCosNet~\cite{zhang2020cross} & 0.977 & 0.958 &  \textbf{0.949}   \\
\midrule
% CoCosNet v2~\cite{zhou2021cocosnet} & \textbf{0.970} & 0.948 &  \multicolumn{2}{c}{0.877}  \\

% MCL-Net~\cite{zhan2022marginal}  & 0.966 & \textbf{0.951} & \multicolumn{2}{c}{\textbf{0.881}}  \\ \hline
MIDMs (Ours)  & \textbf{0.982} & \textbf{0.962} & 0.915    \\
\bottomrule
% \raisebox{2em}{}
% \vspace{-3pt}
\end{tabular}
\end{wraptable} 


==> Table/loss_ablation.tex <==
\begin{table*}[h!]
    \small
    \centering
    \caption{\textbf{Ablation study of each loss function for CelebA-HQ~\cite{liu2015deep}.} (-) denotes the model that trained without the loss function.}\label{table:loss_without} \vspace{-5pt}
        \begin{tabular}{lcc}
        \toprule
        {Loss} & FID $\downarrow$  
        \\
        \midrule
        baseline & \textbf{15.67} \\
        (-) $\mathcal{L}_{\mathrm{cycle}}$ & 16.18  \\
        (-) $\mathcal{L}_{\mathrm{style}}$ & 19.23 \\
        (-) $\mathcal{L}_{\mathrm{perc}}$ & 16.51 \\        
        (-) $\mathcal{L}_{\mathrm{diff}}$ & 17.11 \\
        (-) $\mathcal{L}_{\mathrm{dom}}$ & 16.68 \\
        (-) $\mathcal{L}_{\mathrm{src}}$ & 72.25 \\
        \bottomrule
        \end{tabular}
\end{table*} 


==> Table/table_fid.tex <==
\renewcommand\arraystretch{1.0}
\begin{table*}[h!]
\caption{
\textbf{Additional quantitative evaluation on DeepFashion and CelebA-HQ datasets.}\\ The comparisons are performed with widely used evaluation metrics FID~\cite{heusel2017gans}. FID w.sources is a FID score compared with the distribution of ground-truth images of condition images. FID w.exemplars is a FID score compared with the distribution of exemplar images.
}\label{tab_com}
\vspace{-5pt}
\small
\centering 
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccc} 
\toprule
\multirow{3}[3]{*}{Methods}
& 
\multicolumn{2}{c}{DeepFashion~\cite{liu2016deepfashion} } &
\multicolumn{2}{c}{CelebA-HQ~\cite{liu2015deep}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& FID  $\downarrow$ & FID  $\downarrow$  
& FID  $\downarrow$ & FID  $\downarrow$   
\\
& w. sources & w.exemplars  
& w. sources  & w.exemplars
\\
\midrule
UNITE~\cite{zhan2021unbalanced} & 13.08 & - & 13.15 & - \\
CoCosNet~\cite{zhang2020cross}         & 14.40  & 11.12        & 14.30 & 11.01      \\
CoCosNet v2~\cite{zhou2021cocosnet}        & 12.81  & - & 12.85 & -      \\ 
MCL-Net~\cite{zhan2022marginal}  & 12.89 & - & \textbf{12.52} & -  \\
MIDMs (Ours)         & \textbf{10.89} & \textbf{8.54}   & 15.67 & \textbf{10.67}  \\ 
\bottomrule
\end{tabular} %\vspace{-10pt}
% }
\end{table*}

% Celeb
% src : 15.67 12.34
% ref src randomix : 13.17, 11.29

% DeepFashion


==> figure/fig_comparison.tex <==
\begin{figure*}[t]
    \center
    \small
    \setlength\tabcolsep{1pt}
    {
    \renewcommand{\arraystretch}{0.3}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{cccccccc}
        Condition & Exemplar &  Pix2pixHD &  SPADE &  UNITE  & CoCosNet~\cite{ma2018exemplar} & CoCosNet v2~\cite{ma2018exemplar}  &  Ours \\[0.1ex]
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cond_0.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/ex_0.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/pixpix_0.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/spade_0.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/unite_0.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cocos_0.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cocosv2_0.png} &
        \includegraphics[width=0.15\columnwidth]{figure/qual/ours_0.png} &\\
        % ref: images/training/ADE_train_00015347.jpg cond: ADE_val_00000436.jpg
        
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cond_1.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/ex_1.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/pixpix_1.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/spade_1.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/unite_1.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cocos_1.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cocosv2_1.png} &
        \includegraphics[width=0.15\columnwidth]{figure/qual/ours_1.png} &\\
        
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cond_2.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/ex_2.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/pixpix_2.png} & 
        \includegraphics[width=0.15\columnwidth]{figure/Qual/spade_2.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/unite_2.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cocos_2.png} &
        \includegraphics[width=0.15\columnwidth]{figure/Qual/cocosv2_2.png} &
        \includegraphics[width=0.15\columnwidth]{figure/qual/ours_2.png} &\\
    \end{tabular}
    }}
    \caption{\textbf{
    Qualitative comparison of MIDM and other state-of-the-art image translation method.}}
    \label{fig:comparison} \vspace{-10pt}
\end{figure*}

==> figure/fig_onecond_celeba.tex <==
\begin{figure*}[t]
\centering
\small
% \begin{subfigure}[b]{0.5\textwidth}
\setlength\tabcolsep{0pt}
{
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{@{}rrccccccc@{}}
    &
    \raisebox{0.22\height}{\rotatebox{90}{Exemplars}} \hspace{2pt}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10_r.jpg}&\\
    \raisebox{0.25\height}{\rotatebox{90}{CoCosNet}}\hspace{2pt} &
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/trg.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10.png}\\
    \raisebox{1.05\height}{\rotatebox{90}{Ours}} \hspace{2pt}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/trg.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10_o.jpg}\\
\end{tabular}
}
% \end{subfigure}
\\
\vspace{0.5em}
(a) Edge to face (CelebA-HQ~\cite{liu2015deep})\\
\vspace{0.5em}

\setlength\tabcolsep{0pt}
{
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{@{}rrccccccc@{}}
    &
    \raisebox{0.22\height}{\rotatebox{90}{Exemplars}} \hspace{2pt}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10_r.jpg}&\\
    \raisebox{0.25\height}{\rotatebox{90}{CoCosNet}}\hspace{2pt} &
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/trg.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10.png}\\
    \raisebox{1.05\height}{\rotatebox{90}{Ours}} \hspace{2pt}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/trg.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10_o.jpg}\\
\end{tabular}
}\\
\vspace{0.5em}
(b) Pose to body (DeepFashion~\cite{liu2016deepfashion})\\
\caption{\textbf{Qualitative results with different exemplars:} (from top to bottom) exemplars, condition and results by CoCosNet~\cite{zhang2020cross} and MIDMs (ours).}
\label{figure:cebeba_result} \vspace{-10pt}
\end{figure*}

==> figure/fig_onecond_deepfashion.tex <==
\begin{figure*}[t]
\center
\small
\setlength\tabcolsep{0pt}
{
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{@{}rrccccccc@{}}
    &
    \raisebox{0.22\height}{\rotatebox{90}{Exemplars}}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8_ref.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10_r.jpg}&\\
    \raisebox{0.25\height}{\rotatebox{90}{CoCosNet}}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/trg.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8.png}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10.png}\\
    \raisebox{1.05\height}{\rotatebox{90}{Ours}}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/trg.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/1_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/4_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/6_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/8_o.jpg}&
    \includegraphics[width=0.15\columnwidth]{figure/Celeb/10_o.jpg}\\
\end{tabular}
}
\caption{\textbf{Results with different exemplars in pose to body synthesis (DeepFashion~\cite{liu2016deepfashion}).} (from top to bottom) exemplars, condition and results by CoCosNet~\cite{zhang2020cross} and MIDMs (ours).}
\label{figure:deepfashion_result} \vspace{-10pt}
\end{figure*}

==> figure/fig_style_transfer.tex <==
\begin{figure*}[h]
	\centering
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/3_c.png}
        \caption{Content}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/3_s.png}
        \caption{Style}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/style_transfer.png}
        \caption{}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/swapping.png}
        \caption{}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/cocos.png}
        \caption{}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/sinir_02.png}
        \caption{}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/ditp.png}
        \caption{}
        \end{subfigure}
	\begin{subfigure}[b]{0.120\textwidth}
	\includegraphics[width=1.0\linewidth]{figure/Style/14259.jpg}
        \caption{}
        \end{subfigure}

	\vspace{-5pt}
	\caption{\textbf{Qualitative comparison with state-of-the-art methods on CelebA-HQ~\cite{liu2015deep}.}  Given content (a) and style (b) images, translation results are achieved by (c) Gatys et al.~\cite{gatys2016image}, (d) Swapping Autoencoder~\cite{park2020swapping}, (e) CoCosNet~\cite{zhang2020cross}, (f) SinIR~\cite{yoo2021sinir}, (g) DTP~\cite{kim2021deep}, and (h) our MIDMs. 
	}
	\label{celebahq_result}\vspace{-5pt}
\end{figure*}

==> table/macro.tex <==
% this is from D2C: Diffusion-Decoding Models for Few-Shot Conditional Generation Arxiv LaTeX

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}
\newcommand{\bb}[1]{{\mathbb{#1}}}
\newcommand{\norm}[1]{{\lVert {#1} \rVert}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{Eq.(\ref{#1})}
\def\Eqref#1{Equation~(\ref{#1})}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

\def\tq{{\overline{q}}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}

\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vpsi{{\bm{\psi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vpi{{\bm{\pi}}}
\def\vomega{{\bm{\omega}}}
\def\vlambda{{\bm{\lambda}}}
\def\vtheta{{\bm{\theta}}}
\def\vphi{{\bm{\phi}}}
\def\vmu{{\bm{\mu}}}
\def\Hw{{H_\vomega(\vx)}}
\def\Et{{E_\vtheta(\vx)}}
\def\HE{{\Hw + \Et}}
\newcommand{\at}[2][]{#1|_{#2}}
\def\otheta{{\vtheta^*}}
\def\oomega{{\vomega^*}}
\def\ophi{{\vphi^*}}
\def\vJ{{\bm{J}}}
\def\vK{{\bm{K}}}
\def\vP{{\bm{P}}}
\def\vQ{{\bm{Q}}}
\def\vS{{\bm{S}}}
\def\vU{{\bm{U}}}
\def\vW{{\bm{W}}}
\def\vI{{\bm{I}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\DF}{D_f}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %


\let\ab\allowbreak
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\js}[1]{{\color{teal} [JS: #1]}}
\newcommand{\s}[1]{{\color{magenta} [SE: #1]}}
\newcommand{\se}[1]{{\color{magenta} [SE: #1]}}
\newcommand{\chenlin}[1]{{\color{cyan} [CM: #1]}}
\newcommand{\abhishek}[1]{{\color{red} [Abhishek: #1]}}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\dop}{\mathrm{do}}
\newcommand{\supp}{\mathrm{supp}}

\newcommand{\epsilonv}{\mathbf{\epsilon}}

\newcommand{\gtheta}{g_\theta}
\newcommand{\fphi}{f_\phi}
\newcommand{\ptheta}{p_\theta}
\newcommand{\qphi}{q_\phi}

==> table/main_style_transfer_table.tex <==
\renewcommand\arraystretch{1.0}
\begin{wraptable}{r}{5.0cm}
\vspace{-5mm}
\caption{\textbf{Quantitative evaluation on CelebA-HQ~\cite{liu2015deep}.}} 
\label{tab_styletransfer}
\vspace{-5pt}
\small  
\renewcommand\tabcolsep{8pt}
\centering 
\begin{tabular}{
l|cc
} \hline
Method & 
PE$\downarrow$ &
SSIM$\uparrow$
\\\hline

Gatys et al.~\cite{gatys2016image}  & 4.37 & 0.66 \\
STROTSS~\cite{kolkin2019style}  & 1.81 & 0.60 \\
Swap. AE~\cite{park2020swapping}  & 0.89 & 0.60 \\
CoCosNet~\cite{zhang2020cross} & 1.56 & 0.43 \\
SinIR~\cite{yoo2021sinir}  & 1.56 & 0.84 \\
DTP~\cite{kim2021deep}  & 0.79 & 0.86 \\\hline
MIDMs (Ours)  & \textbf{soon} & \textbf{soon} \\\hline

\end{tabular}\vspace{-10pt}
\end{wraptable} 

